Mitigating Cache Noise in Test-Time Adaptation for Large Vision-Language Models

Test-time adaptation (TTA) of visual language models has recently attracted significant attention as a solution to the performance degradation caused by distribution shifts in downstream tasks. However, existing cache-based TTA methods have certain limitations. They mainly rely on the accuracy of cached feature labels, and the presence of noisy pseudo-labels can cause these features to deviate from their true distribution. This makes cache retrieval methods based on similarity matching highly sensitive to outliers or extreme samples. Moreover, current methods lack effective mechanisms to model class distributions, which limits their ability to fully exploit the potential of cached information. To address these challenges, we introduce a comprehensive and reliable caching mechanism and propose a novel zero-shot TTA method called "Cache, Residual, Gaussian" (CRG). This method not only employs learnable residual parameters to better align positive and negative visual prototypes with text prototypes, thereby optimizing the quality of cached features, but also incorporates Gaussian Discriminant Analysis (GDA) to dynamically model intra-class feature distributions, further mitigating the impact of noisy features. Experimental results on 13 benchmarks demonstrate that CRG outperforms state-of-the-art TTA methods, showcasing exceptional robustness and adaptability.

==> fig/Two_classic_method.tex <==
% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}{0.4\textwidth} % Correct environment: subfigure instead of subcaption
%         \centering
%         \includegraphics[width=\linewidth]{fig/TPT.png}
%         \label{fig:image1}
%     \end{subfigure}\hfill

    
%     \begin{subfigure}{0.5\textwidth} % Correct environment: subfigure instead of subcaption
%         \centering
%         \includegraphics[width=\linewidth]{fig/TDA.png}
%         \label{fig:image2}
%     \end{subfigure}\hfill
%     \caption{Two classic Method of Test Time Adaption}
%     \label{fig:two_classic_method}
% \end{figure}

%底下是竖着的，上面是横着的


\begin{figure}[!ht]
    \centering
    \begin{subfigure}{0.6\textwidth} % Correct environment: subfigure instead of subcaption
        \centering
        \includegraphics[width=\linewidth]{fig/TPT.png}
        \caption{Test-Time Prompt Tuning\cite{TPT}}
        \label{fig:two_classic_method1}
    \end{subfigure}

    \vspace{1em}
    
    \begin{subfigure}{0.8\textwidth} % Correct environment: subfigure instead of subcaption
        \centering
        \includegraphics[width=\linewidth]{fig/TDA.jpg}
        \caption{Training-free Dynamic Adaption\cite{TDA}}
        \label{fig:two_classic_method2}
    \end{subfigure}\hfill
    \caption{Two Classic Method of Test Time Adaption}
    \label{fig:two_classic_method}
\end{figure}


==> fig/cache.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{fig/cache.png}
    \caption{\textbf{Framework Structure of CRG for Zero-Shot Test-time Adaptation} The CRG framework is an extension of CLIP designed for zero-shot online adaptation. It incorporates three cache structures and three learnable residuals, facilitating a comprehensive prediction by integrating features from both CLIP and the cache.}
    %CRG的零样本在线适配框架结构，它基于CLIP扩展而来，包含三个Cache结构，三个可学习的残差，以及融合CLIP和Cache的综合预测
    \label{fig:cache}
    \vspace{-10pt} 
\end{figure}

==> fig/error_and_comparison.tex <==
% \begin{figure}[!ht]
%     \centering
%     \begin{subfigure}{0.24\textwidth} % Correct environment: subfigure instead of subcaption
%         \centering
%         \includegraphics[width=\linewidth]{fig/error_rate_plot.png}
%         \label{fig:image1}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.24\textwidth} % Correct environment: subfigure instead of subcaption
%         \centering
%         \includegraphics[width=\linewidth]{fig/few_vs_zero_performance_bar_chart.png}
%         \label{fig:image2}
%     \end{subfigure}\hfill
%     \caption{Analysis}
%     \label{fig:error_comparison}
% \end{figure}

%底下是竖着的，上面是横着的

\begin{figure}[!ht]
    \centering
    \begin{subfigure}{0.35\textwidth} % 宽度设置为 50% 的页面宽度
        \centering
        \includegraphics[width=\linewidth]{fig/error_rate_plot.png}
        \caption{Error Rate Plot} % 可以添加单独的子图说明
        \label{fig:image1}
    \end{subfigure}

    \vspace{1em} % 添加垂直间距
    \vspace{-5pt} 
    \begin{subfigure}{0.35\textwidth} % 宽度设置为 50% 的页面宽度
        \centering
        \includegraphics[width=\linewidth]{fig/few_vs_zero_performance_bar_chart.png}
        \caption{Few-shot vs Zero-shot } % 子图说明
        \label{fig:image2}
    \end{subfigure}
    \caption{Figure (a) shows the change in error rates for the positive cache during downstream testing with the TDA\cite{TDA} method, while Figure (b) compares the performance gap between similarity-based cache models in zero-shot(TDA\cite{TDA}) and few-shot (Tip-adapter\cite{TipAdapter}) settings, all using RN50 as the backbone.}
    \label{fig:error_comparison}
    \vspace{-15pt} 
\end{figure}


==> tables/supp_ood.tex <==
% \renewcommand\arraystretch{0.9}
\begin{table*}[ht]
\renewcommand\arraystretch{1.0}
\caption{\textbf{Performance comparisons on robustness to natural distribution shifts}. We present top-1 accuracy (\%) results for all evaluated methods employing both ResNet-50 and ViT-B/16 visual backbones of CLIP. Additionally, we assess the performance using prompts learned by CoOp~\cite{zhou2022learning} with 16-shot training data per class on ImageNet~\cite{deng2009imagenet}. The best results are highlighted in \textbf{bold}.}
\vspace{5pt}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lccccccc}
    \toprule
    {Method}      & ImageNet   &  ImageNet-A  &  ImageNet-V2  & ImageNet-R 
    & ImageNet-S   
    &{Average}  & {OOD Average}     \\
  \midrule
  CLIP-ResNet-50~\cite{radford2021learning}       &58.16&	21.83&	51.41	&56.15	&33.37&	44.18&	40.69           \\ 
  \midrule
  Ensemble          &  59.81&	23.24&	52.91	&{60.72}	&35.48&	46.43&	43.09  \\
  TPT~\cite{shu2022test}          &  60.74 & 26.67  &    54.70   &  59.11   &  35.09   &    47.26    &     43.89    \\
  DiffTPT~\cite{feng2023diverse} & 60.80 & \textbf{31.06} & 55.80 & 58.80 & 37.10 & 48.71 & 45.69 \\
  TDA~\cite{karmanov2024efficient} & 61.35 & 30.29 & 55.54 & 62.58 & 38.12 & 49.58 & 46.63 \\ \rowcolor{gray!20}
  \textbf{Ours} & \textbf{63.41} & 30.15 & \textbf{56.72} & \textbf{63.72} & \textbf{40.03} & \textbf{50.81}  & \textbf{47.66} \\ \rowcolor{gray!20}
   & ($\pm$ 0.23) & ($\pm$ 0.41) & ($\pm$ 0.22) & ($\pm$ 0.20) & ($\pm$ 0.11) & ($\pm$ 0.21)  & ($\pm$ 0.22) \\
  \midrule
  CoOp~\cite{zhou2022learning}            &  63.33 &  23.06  &   55.40     &  56.60   &  34.67   &     46.61   &     42.43       \\
    TPT + CoOp~\cite{shu2022test}           &  64.73  & 30.32  & 57.83       &  58.99   &  35.86   &   49.55     &   45.75\\
  DiffTPT + CoOp~\cite{feng2023diverse}           &  64.70  & \textbf{32.96}  & \textbf{61.70}       &  58.20   &  36.80   &   \textbf{50.87}     &   \textbf{47.42} \\ \rowcolor{gray!20}
  % TDA + CoOp$^\dag$~\cite{karmanov2024efficient} & 62.71 & 29.96 & 55.75 & 59.76 & \textbf{38.02} & 49.24 & 45.87 \\ \rowcolor{gray!20}
\textbf{Ours + CoOp} & \textbf{64.86} & 30.08 & 57.96 & \textbf{59.78} & \textbf{37.80} & 50.10 & 46.41 \\ \rowcolor{gray!20}
   & ($\pm$ 0.18) & ($\pm$ 0.27) & ($\pm$ 0.31) & ($\pm$ 0.19) & ($\pm$ 0.17) & ($\pm$ 0.22)  & ($\pm$ 0.23) \\
  \midrule
  \midrule
  CLIP-ViT-B/16~\cite{radford2021learning}       & 66.73&	47.87&	60.86&	73.98&	46.09&	59.11&	57.20             \\
  \midrule
  Ensemble          &  68.34&	49.89&	61.88&	{77.65}&	48.24&	61.20&	59.42  \\
  TPT~\cite{shu2022test}           &  68.98  & 54.77  & 63.45       &  77.06   &  47.94   &   62.44     &   60.81 \\
  DiffTPT~\cite{feng2023diverse}           &  70.30  & 55.68  & 65.10       &  75.00   &  46.80   &   62.28     &   60.52 \\
  TDA~\cite{karmanov2024efficient} & 69.51 & \textbf{60.11} & 64.67 & 80.24 & 50.54 & 65.01 & 63.89 \\ \rowcolor{gray!20}
  \textbf{Ours} & \textbf{71.91} & 59.63 & \textbf{65.44} & \textbf{80.40} & \textbf{52.26} & \textbf{65.93} & \textbf{64.43} \\ \rowcolor{gray!20}
   & ($\pm$ 0.09) & ($\pm$ 0.18) & ($\pm$ 0.17) & ($\pm$ 0.24) & ($\pm$ 0.11) & ($\pm$ 0.16)  & ($\pm$ 0.18) \\
  \midrule
  CoOp~\cite{zhou2022learning}          &  71.51 &  49.71  &   64.20     &  75.21   &  47.99   &   61.72     &   59.28  \\
  TPT + CoOp~\cite{shu2022test}           &  73.61  & 57.95  & \textbf{66.83}       &  77.27   &  49.29   &   64.99     &   62.83 \\
  DiffTPT + CoOp~\cite{feng2023diverse}           &  \textbf{75.00}  & 58.09  & 66.80       &  73.90   &  49.50   &   64.12     &   61.97 \\ \rowcolor{gray!20}
  % TDA + CoOp$^\dag$~\cite{karmanov2024efficient} & 71.13 & \textbf{59.83} & 64.81& \textbf{79.73} & 50.74 & 65.25 &  \\ \rowcolor{gray!20}
\textbf{Ours + CoOp} & 73.67 & \textbf{59.43} & 66.38 & 78.49 & \textbf{50.78} & \textbf{65.75} & \textbf{63.77} \\ \rowcolor{gray!20}
   & ($\pm$ 0.14) & ($\pm$ 0.36) & ($\pm$ 0.32) & ($\pm$ 0.06) & ($\pm$ 0.08) & ($\pm$ 0.23)  & ($\pm$ 0.26) \\
    \bottomrule
  \end{tabular}
    }
\label{tab:ood-supp}
\end{table*}
  

==> tables/supp_others.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%

% \renewcommand\arraystretch{0.95}
\begin{table*}[ht]
  \caption{\textbf{Performance comparisons on cross-datesets generalization.} We also present top-1 accuracy (\%) for all methods on two backbones of CLIP. The best results are highlighted in \textbf{bold}.}
  \vspace{5pt}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lp{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
      \toprule
      Method & Aircraft & Caltech & Cars & DTD & EuroSAT & Flower & Food101 & Pets & SUN397 & UCF101 & Average \\
      \midrule
      CLIP-ResNet-50 & 15.66 & 85.88 & 55.70 & 40.37 & 23.69 & 61.75 & 73.97 & 83.57 & 58.80 & 58.84 & 55.82 \\
      \midrule
      Ensemble & 16.11 & 87.26 & 55.89 & 40.37 & 25.79 & 62.77 & 74.82 & 82.97 & 60.85 & 59.48 & 56.63 \\
      CoOp~\cite{zhou2022learning} & 15.12 & 86.53 & 55.32 & 37.29 & 26.20 & 61.55 & 75.59 & \textbf{87.00} & 58.15 & 59.05 & 56.18 \\
      % CoCoOp~\cite{zhou2022conditional} & 14.61 & 87.38 & 56.22 & 38.53 & 28.73 & 65.57 & 76.20 & \textbf{88.39} & 59.61 & 57.10 & 57.23 \\
      \midrule
      TPT~\cite{shu2022test}  & 17.58 & 87.02 & 58.46 & 40.84 & 28.33 & 62.69 & 74.88 & 84.49 & 61.46 & 60.82 & 57.66 \\
      DiffTPT~\cite{feng2023diverse} & 17.60 & 86.89 & \textbf{60.71} & 40.72 & 41.04 & 63.53 & \textbf{79.21} & 83.40 & 62.72 & 62.67 & 59.85 \\
      TDA~\cite{karmanov2024efficient}  & 17.61 & 89.70 & 57.78 & 43.74 & \textbf{42.11} & \textbf{68.74} & 77.75 & 86.18 & 62.53 & \textbf{64.18}  & 61.03\\ \rowcolor{gray!20}
      \textbf{Ours} & \textbf{19.80} & \textbf{90.83} & 59.25 & \textbf{50.18} & 41.67 & 67.60 & 77.83 & 85.97 & \textbf{64.23} & 61.98 & \textbf{61.93} \\
      \midrule
      \midrule
      CLIP-ViT-B/16 & 23.67 & 93.35 & 65.48 & 44.27 & 42.01 & 67.44 & 83.65 & 88.25 & 62.59 & 65.13 & 63.58 \\
      \midrule
      Ensemble & 23.22 & 93.55 & 66.11 & 45.04 & 50.42 & 66.99 & 82.86 & 86.92 & 65.63 & 65.16 & 64.59 \\
      CoOp~\cite{zhou2022learning} & 18.47 & 93.70 & 64.51 & 41.92 & 46.39 & 68.71 & 85.30 & 89.14 & 64.15 & 66.55 & 63.88 \\
      % CoCoOp~\cite{zhou2022conditional} & 22.29 & 93.79 & 64.90 & 45.45 & 39.23 & 70.85 & 83.97 & 90.46 & 66.89 & 68.44 & 64.63 \\
      \midrule
      TPT~\cite{shu2022test}  & 24.78 & 94.16 & 66.87 & 47.75 & 42.44 & 68.98 & 84.67 & 87.79 & 65.50 & 68.04 & 65.10 \\
      DiffTPT~\cite{feng2023diverse} & 25.60 & 92.49 & 67.01 & 47.00 & 43.13 & 70.10 & \textbf{87.23} & 88.22 & 65.74 & 62.67 &65.47 \\
      TDA~\cite{karmanov2024efficient} & 23.91 & 94.24 & 67.28 
      & 47.40 & \textbf{58.00} & 71.42 & 86.14 & 88.63 & 67.62 & \textbf{70.66} & 67.53 \\ \rowcolor{gray!20}
      \textbf{Ours} & \textbf{28.95} & \textbf{94.81} & \textbf{67.31} & \textbf{54.20} & 55.79 & \textbf{75.07} & 86.17 & \textbf{91.14} & \textbf{70.07} & 70.44 & \textbf{69.40} \\
      \bottomrule
    \end{tabular}
  } 
  \label{tab:fine-grained-supp}
  \vspace{10pt}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
